Local Convergence of Gradient Methods for Min-Max Games: Partial Curvature Generically Suffices

We study the convergence to local Nash equilibria of gradient methods for two-player zero-sum differentiable games. It is well-known that such dynamics converge locally when $S \succ 0$ and may diverge when $S=0$, where $S\succeq 0$ is the symmetric part of the Jacobian at equilibrium that accounts for the "potential" component of the game. We show that these dynamics also converge as soon as $S$ is nonzero (partial curvature) and the eigenvectors of the antisymmetric part $A$ are in general position with respect to the kernel of $S$. We then study the convergence rates when $S \ll A$ and prove that they typically depend on the average of the eigenvalues of $S$, instead of the minimum as an analogy with minimization problems would suggest. To illustrate our results, we consider the problem of computing mixed Nash equilibria of continuous games. We show that, thanks to partial curvature, conic particle methods -- which optimize over both weights and supports of the mixed strategies -- generically converge faster than fixed-support methods. For min-max games, it is thus beneficial to add degrees of freedom "with curvature": this can be interpreted as yet another benefit of over-parameterization.

==> sections/4_particleMNE_bak.tex <==
% !TEX root = ../main.tex
% \documentclass[../main]{subfiles}
%\begin{document}

\section{Illustration: sparse mixed Nash equilibria of continuous games} \label{sec:particleMNE}

The problem of finding the mixed Nash equilibria (MNE) of two-player zero-sum games is a classical one in game theory.
It consists, given 
% (pure) 
strategy spaces $\XXX$, $\YYY$ and a 
% (pure) 
payoff function $f: \XXX \times \YYY \to \RR$, in solving the min-max game
$
    \min_{\mu \in \PPP(\XXX)} \max_{\nu \in \PPP(\YYY)} \EE_{x \sim \mu, y \sim \nu} [f(x, y)]
$,
where $\PPP(\XXX)$ denotes the space of probability measures -- representing mixed strategies -- over $\XXX$.

Consider a two-player zero-sum game where $\XXX$ and $\YYY$ are continuous sets, say, $\XXX=\YYY=\TT^1$ the one-dimensional Euclidean torus,%
\footnote{
    The choice of $\XXX=\YYY=\TT^1$ is made for simplicity of exposition. The discussion below extends straightforwardly to toruses of any dimension,
    and could be extended to $\XXX, \YYY$ Riemannian manifolds without boundaries at the cost of more technical notation.
}
and $f: \TT^1 \times \TT^1 \to \RR$ is smooth.
Assume for simplicity that the MNE $(\mu^*, \nu^*)$ is unique and has finite supports:
$\support(\mu^*) = \left\lbrace x^*_I, 1 \leq I \leq N \right\rbrace$,
$\support(\nu^*) = \left\lbrace y^*_J, 1 \leq J \leq M \right\rbrace$
(this is the case for example if $f$ is a sum of separable functions \citep{stein_separable_2008}).
We consider
two natural algorithms:
\begin{enumerate}[leftmargin=5mm,itemsep=0mm]
    \item If the support points $(x^*_I)_I$, $(y^*_J)_J$ are known, then we may restrict attention to measures supported on those points. The problem reduces to a constrained bilinear game
    \begin{equation} \label{eq:particleMNE:MP_pb}
        \min_{a \in \Delta_N} \max_{b \in \Delta_M} 
        \left\lbrace 
            \EE_{I \sim a, J \sim b} [f(x^*_I, y^*_J)] 
            = \sum_{I=1}^N \sum_{J=1}^N a_I b_J f(x^*_I, y^*_J)
            \eqqcolon a^\top P b
        \right\rbrace
    \end{equation}
    where $\Delta_N \simeq \PPP(\{1,...,N\})$ denotes the standard simplex. We may then apply Mirror Prox (MP) with entropy link function 
    \citep{nemirovski_prox-method_2004}.
    % which corresponds to the Bregman-geometry analog of EG.

    This algorithm converges to the MNE for any small enough $\eta$ with an exponential rate at least proportional to $\eta^2$~\cite{wei_linear_2021}, and this scaling is tight numerically, as visible from the green line in \autoref{fig:particleMNE:rate_vs_eta}.
    \item If only the number of support points is known, we may consider a discretization of the strategy spaces using $N$, resp.\ $M$ points, and optimize over both the discretization points and the probability measures. The problem reduces to
    \begin{equation} \label{eq:particleMNE:CPMP_pb}
        \min_{(a, x) \in \Delta_N \times (\TT^1)^N} ~
        \max_{(b, y) \in \Delta_M \times (\TT^1)^M} ~
        \sum_{I=1}^N \sum_{J=1}^M a_I b_J f(x_I, y_J)
    \end{equation}
    which is nonconvex-nonconcave in general.
    We may then apply an iterative method where 
    the $a, b$ are updated using MP steps with step-size $\eta$ and $x, y$ are updated using EG steps with step-size $\gamma \eta$ for some parameter $\gamma>0$, 
    called Conic Particle Mirror Prox in \cite{wang_exponentially_2022}. Note that the main challenge in that reference is to deal with the case where $N$ and $M$ are unknown via over-parameterization, but
    here we assume they are known
    for the sake of simplicity.

    This algorithm, which we will refer to simply as EG, converges to the MNE for any small enough $\eta$ (and any $\gamma>0$) with an exponential rate at least proportional to $\eta^2$, under some non-degeneracy assumptions \cite[Sec.~3.1]{wang_exponentially_2022}.
    % corresponding essentially to requiring that the problem is locally SC-SC in the variables $(x,y)$.
    In fact, as visible in \autoref{fig:particleMNE:rate_vs_eta}, the convergence rate of EG typically scales as $\eta$ -- a fact which we will explain below.
\end{enumerate}

\begin{figure}[t]
    \vspace{-0.5em}
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
    	\includegraphics[width=\textwidth]{rate_vs_alpha}
        \\[-0.5em]
        \caption{
            Convergence rate $r$ vs.~$\gamma$ (fixed $\eta=10^{-2}$)
        }
        \label{fig:particleMNE:rate_vs_alpha}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
    	\includegraphics[width=\textwidth]{rate_vs_eta}
        \\[-0.5em]
        \caption{
            Convergence rate vs.~$\eta$ (fixed $\gamma=10^{-2}$)
        }
        \label{fig:particleMNE:rate_vs_eta}
    \end{subfigure}
    \caption{Observed local convergence rates $r$ (i.e., $\norm{z^k - z^*} = \Theta((1-r)^k)$) for various conic particle methods using step-size $\eta$ for the weights $(a, b)$ and $\gamma \eta$ for the positions $(x, y)$ and for a fixed random draw of $f$. 
    (left) Fixing $\eta=10^{-2}$, we observe a rate for GF (we plot $\eta\cdot\tilde \mu_\gamma$) scaling as $\gamma^2$ as predicted in~\autoref{prop:particleMNE:scale_gamma2}. Interestingly, Alt-GDA has exactly the same behavior, while the behavior of Sim-GDA and EG differ for small $\gamma$, due to the corrective terms shown in~\autoref{tab:expans}. 
    (right) Fixing $\gamma=10^{-2}$, we observe a rate scaling as $\eta$ and a convergence mostly faster than for $\gamma=0$ (where Mirror Descent-Ascent does not converge and MP's rate scales as $\eta^2$~\cite{wei_linear_2021}).}
    \label{fig:particleMNE:manyalphas}
\end{figure}

In \figureref{fig:particleMNE:manyalphas}, we track the evolution of 
the iterates' distance to the solution $\norm{z^k - z^*}$ 
% the iterates' divergence from the solution $D(z^*, z^k)$
when initialized close to the solution, for a randomly generated payoff function $f$ and for various choices of step-size 
(see 
\ifextended% 
    \appendixref{subsec:details_particleMNE:for_figure} 
\else%
    the Appendix
\fi
% for the definition of $D(z^*, z^k)$ and for the distribution from which $f$ was drawn).
for the distribution from which $f$ was drawn and for the precise definition of $\norm{z^k - z^*}$).
Besides EG, we also show the performance of the analogs of Sim-GDA and Alt-GDA for this problem -- all of which share the same continuous-time flow (``GF'') -- in order to illustrate the insights from \autoref{subsec:quantitative:DT_algos}.

Note from \autoref{fig:particleMNE:rate_vs_eta} that, at least for the particular $f$ and value of $\gamma$ used in this experiment, 
EG converges locally faster than MP for the same $\eta$
(in number of iterations, the per-iteration costs differing only by a constant factor), 
even though the former does not use the knowledge of the support points!

\paragraph{Overparameterization induces partial curvature.}
Let us inspect the ``Jacobians'' at optimum for the two dynamics, MP vs.\ EG with parameter $\gamma$.
Due to the simplex constraints and the non-Euclidean nature of the updates for $a, b$,
the relevant matrices are $M_{\MP}$ and $M_\gamma$ defined below, in the sense that the exponential convergence rate of each algorithm is $\tmu_M \eta + O(\eta^2)$ 
\ifextended%
    (see \appendixref{subsec:details_particleMNE:MP},~\ref{subsec:details_particleMNE:CPMP}).
\else%
    (see the Appendix).
\fi
Namely,
omitting half of the antisymmetric off-diagonals for readability,
\vspace{-0.25em}  % manually tweak vertical spacing to control page break location...
\begin{equation}
\label{eq:particleMNE:tM_MP}
    M_{\MP} 
    = \begin{bmatrix}
        \bmzero & \Pi_a D_a P D_b \Pi_b^\top \\
        -(*)^\top & \bmzero
    \end{bmatrix}
\vspace{-0.25em}  % manually tweak vertical spacing to control page break location...
\end{equation}
where $D_a = \Diag(\sqrt{a^*})$ (square roots being taken component-wise) and
$\Pi_a \in \RR^{(N-1) \times N}$ is any matrix such that $\Pi_a \Pi_a^\top = I_{N-1}$ and $\Pi_a^\top \Pi_a = I_N - \sqrt{a^*} \sqrt{a^*}^\top$,
and likewise for $D_b$ and $\Pi_b \in \RR^{(M-1) \times M}$;
and for EG, 
\vspace{-0.5em}  % manually tweak vertical spacing to control page break location...
\begin{equation}
\label{eq:particleMNE:tM_CPMP}
    M_{\gamma} = \begin{bmatrix}
        \bmzero & \bmzero & \Pi_a D_a P D_b \Pi_b^\top & \sqrt{\gamma} \ \Pi_a D_a [\partial_y P] D_b \\
        \bmzero & \gamma \Diag(\partial_{xx}^2 P b^*) & \sqrt{\gamma} D_a [\partial_x P] D_b \Pi_b^\top & \gamma D_a [\partial_{xy}^2 P] D_b \\
        -(*)^\top & -\left( * \right)^\top & \bmzero & \bmzero \\
        -\left( * \right)^\top & -\left( * \right)^\top & \bmzero & -\gamma \Diag(\partial_{yy}^2 P^\top a^*)
    \end{bmatrix}
\vspace{-0.1em}  % manually tweak vertical spacing to control page break location...
\end{equation}
where 
$\left[ \partial_x P \right]_{IJ} = \partial_x f(x^*_I, y^*_J)$, and likewise for $\partial_y P$, $\partial_{xx}^2 P$, $\partial_{yy}^2 P$, $\partial_{xy}^2 P$.

For MP, it is clear that the equivalent conditions of \theoremref{thm:quadr:eigvals} are violated for any payoff function $f$, and so $\tmu_{M_{\MP}} = 0$.
For EG, depending on $f$ and $\gamma$, they may or may not be violated.
For all of the random payoff functions we considered in our experiments, we observed that $\tmu_{M_{\gamma}} > 0$, suggesting that the conditions hold generically.
They are violated for certain $f$'s however, as shown in
\ifextended%
    \appendixref{subsec:details_particleMNE:counter_example}, 
\else%
    the Appendix,
\fi
so that the scaling in $\eta^2$ of the convergence rate proved in~\cite[Sec.~3.1]{wang_exponentially_2022} is tight in the worst case.
 
More precisely as we show in the next proposition, assuming that the blocks of $M_{\gamma}$ are in general position, we expect $\tmu_{M_{\gamma}}$ to scale as $\gamma^2$, which is indeed observed in the numerical experiment reported in \autoref{fig:particleMNE:rate_vs_alpha}.
The proof, placed in 
\ifextended%
    \autoref{subsec:details_particleMNE:proof_scale_gamma2}, 
\else%
    the Appendix,
\fi
relies on the same tools as \autoref{prop:quantitative:ord1}, that is, on the asymptotic expansions of the eigenvalues of perturbed matrices.

\begin{restatable}{proposition}{particleMNEscaleGammaSq}
% \begin{proposition} 
\label{prop:particleMNE:scale_gamma2}
    Let $S_2$ symmetric and $A_0, A_1, A_2$ antisymmetric real matrices of the form
    {\small{
    \begin{equation*}
        S_2 = \left[
            \begin{array}{c c|c c}
                \bmzero & & & \\
                & * & & \\
                \hline
                & & \bmzero & \\
                & & & *
            \end{array}
        \right],~
        A_0 = \left[
            \begin{array}{c c|c c}
                & & * & \bmzero \\
                & & \bmzero & \bmzero \\
                \hline
                * & \bmzero & & \\
                \bmzero & \bmzero & &
            \end{array}
        \right],~
        A_1 = \left[
            \begin{array}{c c|c c}
                & & \bmzero & * \\
                & & * & \bmzero \\
                \hline
                \bmzero & * & & \\
                * & \bmzero & &
            \end{array}
        \right],~
        A_2 = \left[
            \begin{array}{c c|c c}
                & & \bmzero & \bmzero \\
                & & \bmzero & * \\
                \hline
                \bmzero & \bmzero & & \\
                \bmzero & * & &
            \end{array}
        \right]
    \end{equation*}
    }}%
    and $M_\gamma = \gamma S_2 + A_0 + \sqrt{\gamma} A_1 + \gamma A_2$ for all $\gamma>0$.
    Then $\tmu_{M_\gamma} = O(\gamma^2)$ as $\gamma \to 0$.
% 
    % Assuming the coefficients of $S_2$, $A_0$, $A_1$, $A_2$ are in general position,
    % then $\tmu_{M_\gamma} \sim c \gamma^2$ for some $c>0$ as $\gamma \to 0$.
% \end{proposition}
\end{restatable}

% \end{document}

